Global Average Feature Augmentation for Robust Semantic Segmentation with Transformers

Robustness to out-of-distribution data is crucial for deploying modern neural networks. Recently, Vision Transformers, such as SegFormer for semantic segmentation, have shown impressive robustness to visual corruptions like blur or noise affecting the acquisition device. In this paper, we propose Channel Wise Feature Augmentation (CWFA), a simple yet efficient feature augmentation technique to improve the robustness of Vision Transformers for semantic segmentation. CWFA applies a globally estimated perturbation per encoder with minimal compute overhead during training. Extensive evaluations on Cityscapes and ADE20K, with three state-of-the-art Vision Transformer architectures : SegFormer, Swin Transformer, and Twins demonstrate that CWFA-enhanced models significantly improve robustness without affecting clean data performance. For instance, on Cityscapes, a CWFA-augmented SegFormer-B1 model yields up to 27.7% mIoU robustness gain on impulse noise compared to the non-augmented SegFormer-B1. Furthermore, CWFA-augmented SegFormer-B5 achieves a new state-of-the-art 84.3% retention rate, a 0.7% improvement over the recently published FAN+STL.

==> CWFA_CVPR_FORMAT/tables/large_sota.tex <==
\begin{table}[!t]
    \caption{\textbf{Cityscapes}. Comparison to other methods for large models on Cityscapes and Cityscapes-C.}
    \vspace{-0.25cm}
\begin{minipage}[c]{\columnwidth}
\centering
    \label{tab:sota_cityscape_c}  
\resizebox{0.75\columnwidth}{!}{%
    \begin{tabular}{l|cccc}
    Model  &  Encoder Size   & City       & City-C    &  Retention 
    \\
    \midrule
    DeepLabv3+ (R50)~\cite{kamann2020benchmarking}  &  25.4M  & 76.6 &  36.8  & 48.0\% 
     \\ 
    DeepLabv3+ (R101)~\cite{kamann2020benchmarking}  &  47.9M  & 77.1 &  39.4  &  51.1\%
     \\ 
    DeepLabv3+ (X65)~\cite{kamann2020benchmarking}  & 22.8M  & 78.4 &  42.7  &  54.5\%
     \\ 
    DeepLabv3+ (X71)~\cite{kamann2020benchmarking}  & -  & 78.6 &  42.5  &  54.1\%
     \\ 
     \midrule
    ICNet (\cite{zhao2018icnet})  &  -  & 65.9 &  28.0  & 42.5\% 
     \\ 
         FCN8s (\cite{long2015fully})  &  50.1M  & 66.7 &  27.4  & 41.1\% 
     \\ 
         DilatedNet (\cite{yu2015multi})  &  -  & 68.6 &  30.3  &  44.2\%
     \\ 
         ResNet38 (\cite{wu2019wider})  &  -  & 77.5 &  32.6  &  42.1\% 
     \\ 
         PSPNet (\cite{zhao2017pyramid})  &  13.7M  & 78.8 &  34.5  &  43.8\%
     \\ 
         ConvNeXt-T (\cite{liu2022convnet})  &  29.0M  & 79.0 &  54.4  &  68.9\% 
     \\ 
     \midrule
         SETR (\cite{heo2021rethinking}) &  22.1M  & 76.0 &  55.3  & 72.8\%  
     \\ 
         SWIN-T (\cite{liu2021swin})  &  28.4M  & 78.1 &  47.3  &  60.6\%
     \\ 
         SegFormer-B0 (\cite{xie2021segformer})  &  3.4M  & 76.2 &  48.8  &  64.0\%
     \\ 
         SegFormer-B1 (\cite{xie2021segformer})  & 13.1M  & 78.4 &  52.7  &  67.2\%
     \\
        SegFormer-B2 (\cite{xie2021segformer})  &  24.2M  & 81.0 &  59.6  &  73.6\%
     \\ 
         SegFormer-B5 (\cite{xie2021segformer})  &  81.4M  & 82.4 &  65.8  &  79.9\%
     \\ 
         SegFormer-B5\footnote{Our reproduced results} (\cite{xie2021segformer})  &  81.4M  & 82.4 &  66.7  &  80.9\% \\ 
      \midrule
        FAN-B-Hybrid~\cite{zhou2022understanding}   &  50.4M  & 82.2 &  66.9  &  81.5\% \\
        FAN-L-Hybrid~\cite{zhou2022understanding}   & 76.8M &  82.3  & 68.7   & {83.5\%}      \\
        \midrule
        \midrule
        STL (FAN-B-Hybrid)~\cite{fan2}   &  50.9M  & 82.5 &  68.6  & 83.2 \% \\
        STL (FAN-L-Hybrid)~\cite{fan2}   & 77.3M &  \textbf{82.8}  &  69.2& {83.6\%}      \\
        \midrule
        Ours: SegFormer B3+CWFA   & 44.0M &  {81.5}  & 68.2  &  83.7\%   \\ 
        Ours: SegFormer B5+CWFA   & 81.4M &  {82.2}  & \textbf{ 69.3}  & \textbf{ 84.3\% }  \\ 
    \end{tabular}
    }  
\end{minipage}
\vspace{-0.5cm}
\end{table}

==> CWFA_CVPR_FORMAT/tables/main_cityscapes.tex <==
\begin{table*}[!t]
\caption{\textbf{Segformer on Cityscapes.} Our results compared to the Segformer baseline. Our approach yields impressive improvements for most corruptions independently of the model size.\AL{mCE is used in classification robustness as mean corruption Error and the definition is slightly different to the mean over corruptions, maybe this could cause confusion?}}
\vspace{-0.5cm}
\label{table: segformer on cityscapes-c}
\scalebox{0.55}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
   \multicolumn{1}{c|}{Model /}& \multirow{2}{*}{Method} & City &\multicolumn{4}{|c|}{Blur}  & \multicolumn{4}{|c|}{Noise} & \multicolumn{4}{|c|}{Digital} & \multicolumn{4}{|c|}{Weather} & \multirow{2}{*}{Average} & \multirow{2}{*}{Reten.}  \\
  \cline{4-19}
    \multicolumn{1}{c|}{Params. [M.]} & &(Clean) & Motion & Defoc & Glass & Gauss & Gauss & Impul & Shot & Speck & Bright & Contr & Satur & JPEG & Snow & Spatt & Fog & Frost & & \\
     \hline
%  \multirow{1}{*}{B0}  & Segformer & \multirow{2}{*}{3.7} & 76.4 & 60.4 & 60.1 & 51.6 & 60.2 & 29.5 & 31.2 & 35.1 & 53.1 & 73.5 & 67.1 & 71.8 & 39.2 & 23.0 & 54.2 & 65.4 & 32.4 & 50.5 & 66.1\\
%  \cline{2-2}\cline{4-22}
% &CWFA (Ours) &  & 75.6 & 61.6 & 60.0 & 57.2 & 60.7 & 44.2 & 46.2 & 49.8 & 61.6 & 73.2 & 66.8 & 70.9 & 44.2 & 38.4 & 60.9 & 64.9 & 41.1 & 56.3 & 74.5 \\
%  \hline
    \multirow{2}{*}{B0 / 3.4}  & Segformer &  76.3 & 59.8 & 59.1 & 51.0 & 59.2 & 25.3 & 27.0 & 30.7 & 51.5 & 73.4 & 66.5 & 72.0 & 38.3 & 22.4 & 53.5 & 65.6 & 31.6 & 49.2 & 64.5\\
  \cline{2-21}
 &CWFA (Ours) & 75.6 & 61.6 & 60.0 & 57.2 & 60.7 & 44.2 & 46.2 & 49.8 & 61.6 & 73.2 & 66.8 & 70.9 & 44.2 & 38.4 & 60.9 & 64.9 & 41.1 & 56.3 & 74.5 \\
 \hline
    \multirow{2}{*}{B1 / 13.1}  & Segformer & 78.5 & 63.9 & 63.7 & 52.2 & 63.7 & 30.2 & 23.7 & 35.8 & 56.3 & 76.4 & 71.0 & 74.9 & 36.7 & 28.3 & 60.4 & 70.8 & 36.7 & 52.8 & 67.2 \\
\cline{2-21}
& CWFA (Ours) & 77.2 & 64.5 & 63.3 & 59.8 & 63.8 & 49.0 & 46.4 & 54.4 & 63.3 & 74.2 & 68.6 & 73.3 & 46.0 & 45.5 & 65.3 & 67.0 & 43.0 & 59.2 & 76.7 \\
  \hline
    \multirow{2}{*}{B2 / 24.2}  & Segformer & 81.0 & 67.7 & 67.8 & 58.6 & 68.3 & 35.8 & 35.6 & 41.4 & 60.3 & 79.7 & 75.6 & 78.4 & 46.0 & 35.0 & 65.4 & 75.7 & 41.3 & 58.3 & 72.0 \\
\cline{2-21}
&CWFA (Ours)  & 80.8 & 69.4 & 68.5 & 63.8 & 69.0 & 55.6 & 55.0 & 61.6 & 71.1 & 79.8 & 74.6 & 78.3 & 50.1 & 52.0 & 70.0 & 74.4 & 50.4 & 65.2 & 80.7 \\
\hline
  \multirow{2}{*}{B3 / 44.0}  & Segformer  &  80.9 & 67.6 & 66.9 & 59.9 & 67.9 & 49.6 & 43.6 & 54.0 & 65.8 & 79.7 & 75.5 & 78.6 & 49.4 & 32.3 & 63.5 & 75.6 & 42.1 & 60.7 & 75.1 \\ 
\cline{2-21}
&CWFA (Ours) &  81.6 & 71.2 & 70.5 & 64.8 & 71.7 & 61.7 & 61.3 & 66.8 & 74.3 & 80.4 & 76.8 & 79.3 & 53.9 & 52.0 & 70.2 & 76.4 & 54.0 & 67.8 & 83.1\\
\hline
  \multirow{2}{*}{B4 / 60.8}  & Segformer & 82.6 & 68.7 & 68.6 & 62.4 & 69.4 & 57.9 & 57.1 & 62.5 & 71.3 & 81.3 & 77.6 & 80.5 & 58.5 & 36.5 & 68.0 & 78.2 & 48.5 & 65.4 & 79.2 \\
\cline{2-21}
&CWFA (Ours) &  81.9 & 70.8 & 70.2 & 64.8 & 71.2 & 61.8 & 60.8 & 67.4 & 74.3 & 80.8 & 77.4 & 79.9 & 56.2 & 50.2 & 70.3 & 77.4 & 52.8 & 67.9 & 82.9 \\
\hline
  \multirow{2}{*}{B5 / 81.4}  & Segformer & 82.4 & 70.4 & 69.4 & 64.8 & 70.3 & 60.2 & 55.2 & 65.4 & 73.5 & 81.3 & 77.7 & 80.4 & 58.9 & 43.1 & 68.9 & 78.6 & 48.7 & 66.7 & 80.9  \\
 \cline{2-21}
 &CWFA (Ours)  & 82.2 & 72.0 & 71.6 & 66.5 & 72.5 & 65.8 & 64.4 & 70.4 & 75.8 & 80.0 & 77.8 & 80.0 & 59.0 & 54.7 & 70.9 & 78.0 & 54.8 & 69.7 & 84.8 \\
\end{tabular}}
\vspace{-0.5cm}
\end{table*}

==> CWFA_CVPR_FORMAT/tables/main_swin_twins.tex <==
\begin{table*}[!t]
\caption{\textbf{Segformer on Cityscapes.} Our results compared to the Segformer baseline. Our approach yields impressive improvements for most corruptions independently of the model size.}
\label{table: segformer on cityscapes-c 160k}
\scalebox{0.55}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
   \multicolumn{1}{c|}{Model /}& \multirow{2}{*}{Method} & City &\multicolumn{4}{|c|}{Blur}  & \multicolumn{4}{|c|}{Noise} & \multicolumn{4}{|c|}{Digital} & \multicolumn{4}{|c|}{Weather} & \multirow{2}{*}{Average} & \multirow{2}{*}{Reten.}  \\
  \cline{4-19}
    \multicolumn{1}{c|}{Params. [M.]} & &(Clean) & Motion & Defoc & Glass & Gauss & Gauss & Impul & Shot & Speck & Bright & Contr & Satur & JPEG & Snow & Spatt & Fog & Frost & & \\
     \hline
%  \multirow{1}{*}{B0}  & Segformer & \multirow{2}{*}{3.7} & 76.4 & 60.4 & 60.1 & 51.6 & 60.2 & 29.5 & 31.2 & 35.1 & 53.1 & 73.5 & 67.1 & 71.8 & 39.2 & 23.0 & 54.2 & 65.4 & 32.4 & 50.5 & 66.1\\
%  \cline{2-2}\cline{4-22}
% &CWFA (Ours) &  & 75.6 & 61.6 & 60.0 & 57.2 & 60.7 & 44.2 & 46.2 & 49.8 & 61.6 & 73.2 & 66.8 & 70.9 & 44.2 & 38.4 & 60.9 & 64.9 & 41.1 & 56.3 & 74.5 \\
%  \hline
    \multirow{2}{*}{Tiny/60}  & Swin & 80.0 & 62.3 & 59.3 & 44.4 & 60.3 & 36.0 & 37.1 & 42.4 & 55.7 & 77.8 & 62.6 & 76.8 & 35.6 & 18.9 & 56.0 & 72.9 & 28.5 & 51.7 & 64.5 \\
    
 & CWFA (Ours) & 79.6 & \textbf{62.4} & \textbf{60.5} & \textbf{47.3} & \textbf{61.7} & \textbf{41.1} & \textbf{44.2} & \textbf{45.6} & 50.4 & 77.2 & 62.1 & 74.4 & \textbf{37.9} & \textbf{26.9} & 52.4 & 72.2 & \textbf{29.1} & \textbf{52.8} & \textbf{66.3} \\
 \hline
    \multirow{2}{*}{Small/ 28.4}  &  Twins-PCPVT & 79.5 & 63.4 & 64.0 & 52.7 & 64.3 & 38.0 & 22.4 & 42.4 & 55.8 & 78.1 & 71.7 & 77.3 & 38.4 & 24.4 & 50.1 & 70.3 & 34.1 & 53.0 & 66.6\\

& CWFA (Ours) & \textbf{79.6} & \textbf{65.9} & \textbf{64.7} & \textbf{58.0} & \textbf{65.3} & \textbf{50.1} & \textbf{35.2} & \textbf{56.1} & \textbf{66.9} & 78.1 & \textbf{72.0} & 77.0 & \textbf{45.8} & \textbf{37.0} & \textbf{59.4} & 69.1 & \textbf{41.6} & \textbf{58.9} & \textbf{73.9} \\
  \hline
    \multirow{2}{*}{Small / 28.3}  & Twins-SVT & 80.9 & 66.9 & 66.8 & 59.4 & 67.4 & 49.6 & 39.4 & 54.1 & 63.4 & 79.6 & 73.9 & 78.1 & 46.2 & 31.8 & 58.8 & 73.5 & 40.3 & 59.3 & 73.3 \\

&  CWFA (Ours)  & -2.0 & \textbf{0.5} & -0.2 & \textbf{2.6} & \textbf{0.1} & \textbf{5.0} & \textbf{11.1} & \textbf{6.1} & \textbf{4.2} & -2.1 & -2.3 & -1.6 & \textbf{5.1} & \textbf{17.8} & \textbf{7.4} & -2.2 & \textbf{7.5} & \textbf{3.7} & \textbf{6.6}\\

\end{tabular}}
\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

